VINE -- A numerical code for simulating astrophysical systems using particles II: Implementation and performance characteristics

We continue our presentation of VINE. We begin with a description of relevant architectural properties of the serial and shared memory parallel computers on which VINE is intended to run, and describe their influences on the design of the code itself. We continue with a detailed description of a number of optimizations made to the layout of the particle data in memory and to our implementation of a binary tree used to access that data for use in gravitational force calculations and searches for SPH neighbor particles. We describe modifications to the code necessary to obtain forces efficiently from special purpose `GRAPE' hardware. We conclude with an extensive series of performance tests, which demonstrate that the code can be run efficiently and without modification in serial on small workstations or in parallel using OpenMP compiler directives on large scale, shared memory parallel machines. We analyze the effects of the code optimizations and estimate that they improve its overall performance by more than an order of magnitude over that obtained by many other tree codes. Scaled parallel performance of the gravity and SPH calculations, together the most costly components of most simulations, is nearly linear up to maximum machine sizes available to us (120 processors on an Origin~3000). At similar accuracy, performance of VINE, used in GRAPE-tree mode, is approximately a factor two slower than that of VINE, used in host-only mode. Optimizations of the GRAPE/host communications could improve the speed by as much as a factor of three, but have not yet been implemented in VINE.

==> vineSRC/vine1.0.7/base/src/makefile <==
#-------------------------------------------------------------------
# makefile for use with GNU make, to make vine.  
#-------------------------------------------------------------------
#-------------------------------------------------------------------
# This module is a component of VINE, copyright by the authors,    #
# as listed below. Please see the COPYING and LICENSE files        #
# in the parent directory for additional information.              #
# This notification is present as an attempt to follow the         #
# recommendations for licensing published on the FSF page.         # 
#-------------------------------------------------------------------


# Here is a list of the possible flags for the making of VINE. Most of 
# the flags are for simply enabling or disabling a feature, i.e. the flag
# is either set to 1 or 0, respectively. For those flags which have additional
# choices, these are explained below with the description of the flag.
#
#   MACHINE   : Select the architecture for which vine will be compiled.
#               Possible choices are as follows. Note that for intel/amd
#               chips, the definition parses to <compiler><chip>:
#
#               PGFAMD64     AMD64 CPUs, use of Portland Group Compiler
#               PATHAMD64    AMD64 CPUs, use of Pathscale Compiler
#               LAHEYAMD     AMD   CPUs, use of Lahey 32bit compiler
#               INTLPGF      Intel CPUs, use of Portland Group Compiler
#               INTLX86      Intel 32bit CPUs, use of Intel Fortran Compiler
#               INTLITAN     Intel Itanium CPUs, use of Intel Fortran Compiler
#               INTLC2DUO    Intel Core 2 Duo, use of Intel Fortran Compiler
#               INTLAMD64    AMD   64bit CPUs, use of Intel Fortran Compiler
#               IBM4         IBM power4 CPUs, like in IBM p690
#               IBM5L        IBM power5 CPUs, like in IBM p570, Linux
#               IBM5A        IBM power5 CPUs, like in IBM p570, AIX
#               G95          Use the g95 compiler 
#               GFORT        Use the gfortan/gcc compiler 
#               G5_P         PowerPC chips in Apple G5 with xlf compiler
#               G5_I         Intel chips in Apple G5 (not currently implemented)
#               SGI          SGI/MIPS R1x000 CPUs, like in SGI Origin
#               SUN          Sun Ultrasparc, like in Sunblade
#               HITACHI      Hitachi SR-8000 CPUs
#
#   MODE      : This flag selects the compiler flags used. Set to FAST for 
#               production runs or DEBUG for debugging. 
#   PARALLEL  : Compile code for running in parallel using OpenMP
#   NDIM      : Number of dimensions. set to value 2 or 3
#   INTEG     : Use the Runge-Kutta integrator (set to RK) or the leapfrog
#               integrator (set to LF). If you write another integrator, 
#               give it a flag.
#   SELFFORCE : Include routines to do self force calculations. 
#               Currently, this means gravity, but you could put
#               something else in instead.
#               Because of some ridiculous LANL copyright nonsense, the forcedirect.F
#               module is distributed as an addon in a different directory
#               Read the file INCLUDE/makefile.dirsum for instructions how to
#               access it.
#   GRAPE     : Allow use of Grape hardware. Set to 
#                    0    for no GRAPE 
#                    3    for GRAPE-3
#                    5    for GRAPE-5
#                    565  for GRAPE-6A using grape5 emulation calls in libg65 (doesn't work)
#                    6    for GRAPE-6
#                    65   for GRAPE-6A using reduced communication libg65 (doesn't work)
#                    66   for GRAPE-6A    
#               Add FAKE to each option above, to use the fakegrape
#               module instead of a real grape. In other words, do
#                    66FAKE to get fakegrape G6A
#               Because of some ridiculous LANL copyright nonsense, the fakegrape
#               module is distributed as an addon in a different directory
#               Read the file INCLUDE/makefile.fakegrape for instructions how to
#               access it.
#
#   SPH       : Use sph subroutines
#   KERNEL    : Which kernel to use for SPH calculations.
#                    currently implement either W4 or W4ALT
#               Because of some ridiculous LANL copyright nonsense, the W4ALT
#               kernel is distributed as an addon module in a different directory
#               Read the file INCLUDE/makefile.altkern for instructions how to
#               access it.
#   PM        : Include point mass subroutines 
#   COSMO     : Use cosmology subroutines
#   PERIODIC  : Use periodic boundary conditions 
#   IOFMT     : Kind of IO to use:
#                       FTNSTD uses only fortran standard io
#                       FXDR uses the xdr library for dump portability
#                       HDF5 add someday 
#   FFTW      : Use the FFTW library for the Fourier transforms of the 
#               periodic boundary conditions (Ewald method)
#   RECIPES   : Include Numerical Recipes routines. Required for some
#               modules to compile, but not included in vine due to
#               copyright restrictions. You can get them yourself easily 
#               enough however.

MACHINE   = G5_P
REAL      = 8
MODE      = FAST
PARALLEL  = 1
NDIM      = 3
INTEG     = LF
SELFFORCE = 1
GRAPE     = 0
SPH       = 1
KERNEL    = W4
PM        = 1
COSMO     = 0
PERIODIC  = 0
FFTW      = 0            #an override sets FFTW=1 if PERIODIC=1
IOFMT     = FTNSTD
RECIPES   = 0

EXEC  = vine107

########################################################################
#
# First strip trailing whitespaces from the definitions above because
# those might mess up the comparisons below.
#
########################################################################

MACHINE   := $(strip $(MACHINE))
REAL      := $(strip $(REAL))
MODE      := $(strip $(MODE))
PARALLEL  := $(strip $(PARALLEL))
NDIM      := $(strip $(NDIM))
INTEG     := $(strip $(INTEG))
SELFFORCE := $(strip $(SELFFORCE))
GRAPE     := $(strip $(GRAPE))
SPH       := $(strip $(SPH))
KERNEL    := $(strip $(KERNEL))
PM        := $(strip $(PM))
COSMO     := $(strip $(COSMO))
PERIODIC  := $(strip $(PERIODIC))
FFTW      := $(strip $(FFTW))
IOFMT     := $(strip $(IOFMT))
########################################################################
#
# Now the flags set above are translated into the appropriate choice of
# preprocessor flags, source files and libraries to link.
#
#######################################################################
#######################################################################
# Type of floating point numbers to use by default

ifeq ($(REAL),4)
   REALCPP = -DREALTYPE=4
else

ifeq ($(REAL),8)
   REALCPP = -DREALTYPE=8
else
   Invalid real type in makefile. Fixme!
endif
endif

#######################################################################
# Dimensions of the code

ifeq ($(NDIM),3)
   NDIMCPP = -DNDIM=3
endif

ifeq ($(NDIM),2)
   NDIMCPP= -DNDIM=2
endif

#######################################################################

# Choice of integrator

ifeq ($(INTEG),RK)
   INTEGCPP = -DRK
   INTEGSRCS = rk12.F
endif

ifeq ($(INTEG),LF)
   INTEGCPP = -DLF
   INTEGSRCS = leapfrog.F
endif

#######################################################################

# Include self forces (e.g. gravity) code

ifeq ($(SELFFORCE),1)

   SELFFORCECPP = -DSELFFORCE
   SELFFORCESRC = forcelaw.F

# GRAPE hardware (assumes real hardware is available 
#  unless make.fakegrape is included. It sets FAKE=1)

   FAKE = 0

   ifeq ($(GRAPE),3)
      GRAPECPP    = -DGRAPE=3 
      GRAPESRC    = grape3.F
      LIBGRAPE    = -lnsl -lgrape3a 
      LDGRAPEPATH = 
   endif

   ifeq ($(GRAPE),5)
      GRAPECPP = -DGRAPE=5
      GRAPESRC = grape5.F 
      ifeq ($(PARALLEL),0)
         LIBGRAPE    = -lg5a -lphibdma
         LDGRAPEPATH = 
      else
         LIBGRAPE    = -lg5ap -lphibdmap
         LDGRAPEPATH = 
      endif
   endif

   ifeq ($(GRAPE),565)
      GRAPECPP    = -DGRAPE=565 -D__LANGUAGE_FORTRAN__
      GRAPESRC    = grape5.F 
      LIBGRAPE    = -lg65
      LDGRAPEPATH = -L/usr/local/g6a
      LDGRAPEPATH = -L.
   endif

   ifeq ($(GRAPE),6)
      GRAPECPP    = -DGRAPE=6 
      GRAPESRC    = grape6.F 
      LIBGRAPE    = -lg6lx
      LDGRAPEPATH = 
   endif

   ifeq ($(GRAPE),65)
      GRAPECPP    = -DGRAPE=65 
      GRAPESRC    = grape6.F 
      LIBGRAPE    = -lg65
      LDGRAPEPATH = -L/usr/local/g6a
   endif

   ifeq ($(GRAPE),66)
      GRAPECPP    = -DGRAPE=66 
      GRAPESRC    = grape6.F 
      LIBGRAPE    = -lg6a
      LDGRAPEPATH = -L/usr/local/g6a
   endif

   include INCLUDE/make.fakegrape
   FAKE := $(strip $(FAKE))

   include INCLUDE/make.dirsum

   SELFFORCECPP += $(GRAPECPP) $(DIRSUMCPP)
   SELFFORCESRC += $(GRAPESRC) $(DIRSUMSRC)
endif

#######################################################################

# Include hydro (SPH)

ifeq ($(SPH),1)
   SPHCPP = -DSPH
   SPHSRC = sph.F eostate.F energy.F
   ifeq ($(KERNEL),W4)
      SPHCPP   += -DW4KERN
      KERNELSRC = W4kern.F
   endif
   include INCLUDE/make.altkern

   SPHSRC += $(KERNELSRC)
endif

#######################################################################

# Include point masses

ifeq ($(PM),1)

   PMCPP   = -DPM
   PMCALC  = pm.F pmcalcs.F

   PMSRCS := $(PMCALC)
endif

#######################################################################

# Periodic boundary conditions

ifeq ($(PERIODIC),1)
   PERIODICCPP = -DPERIODIC
   PERIODICSRC = ewald.F
   FFTW = 1
   FFTW := $(strip $(FFTW))
endif

#######################################################################

# Use of FFTW library

ifeq ($(FFTW),1)
    FFTWCPP = -DFFTW
    ifeq ($(PARALLEL),0)
      LIBFFTW = -lfftw3
   else
      LIBFFTW = -lfftw3_threads -lfftw3
   endif
endif

#######################################################################

# Cosmological expansion

ifeq ($(COSMO),1)
   COSMOCPP = -DCOSMO
   COSMOSRC = cosmo.F 
endif

#######################################################################

# Kind of IO format to include. (Can always do fortran io)

ifeq ($(IOFMT),FTNSTD)
   IOCPP   = 
   LIBIO   = 
   LIOPATH = 
endif
ifeq ($(IOFMT),FXDR)
   IOCPP   = -DXDR
   LIBIO   = -lfxdr
   LIOPATH = -L$(HOME)/local/$(ARCH)/lib
endif

#######################################################################

# Include Numerical Recipes routines 
# (not included in VINE due to copyright--create your own copy as needed)

ifeq ($(RECIPES),1)
   RECIPESCPP = -DRECIPES 
   RECIPESSRC = recipes.f90
endif


######################################################################
#
# Now assemble the preprocessor flags for compiling VINE according to
# the variables set above.
#
######################################################################

PREPROCFLAGS= $(REALCPP) $(NDIMCPP) $(INTEGCPP) $(PERIODICCPP) $(FFTWCPP) \
              $(SELFFORCECPP) $(IOCPP) $(COSMOCPP) $(SPHCPP) $(PMCPP) \
              $(RECIPESCPP)


# Note: we don't use the CPPFLAGS make variable, because we
# want to prefer the fortran preprocessor if one exists


#######################################################################
#
# Choose the compiler and compilation flags for the given machine type
# and run mode (fast = production, debug = debugging)
#
# Add your own compiler here, in the same format if you run on
# different machines that we have listed.
#
#######################################################################

########################
# Power like chips     #
########################

ifeq ($(MACHINE),G5_P)
   include INCLUDE/makefile.g5
endif

ifeq ($(MACHINE),IBM4)
   include INCLUDE/makefile.pwr4
endif

ifeq ($(MACHINE),IBM5L)
   include INCLUDE/makefile.pwr5
endif

########################
# SGI/Mips chips       #
########################

ifeq ($(MACHINE),SGI)
   include INCLUDE/makefile.sgi
endif


########################
# Sun/Sparc chips      #
########################

ifeq ($(MACHINE),SUN)
   include INCLUDE/makefile.sun
endif


########################
# x86 chips            #
########################

ifeq ($(MACHINE),INTLX86)
   include INCLUDE/makefile.x86intl
endif


########################
# x86_64/EMT64 chips   #
########################

ifeq ($(MACHINE),INTLPGF)
   include INCLUDE/makefile.x86pgf
endif

ifeq ($(MACHINE),G95)
   include INCLUDE/makefile.g95
endif

ifeq ($(MACHINE),GFORT)
   include INCLUDE/makefile.gfort
endif

ifeq ($(MACHINE),INTLAMD64)
   include INCLUDE/makefile.amdintl
endif

ifeq ($(MACHINE),PATHAMD64)
   include INCLUDE/makefile.amdpath
endif

ifeq ($(MACHINE),PGFAMD64)
   include INCLUDE/makefile.amdpgf
endif

ifeq ($(MACHINE),LAHEYAMD)
   include INCLUDE/makefile.amdlahey
endif

########################
# Itanic chips         #
########################

ifeq ($(MACHINE),INTLITAN)
   include INCLUDE/makefile.itan
endif

########################
# Core 2 Duo chips     #
########################

ifeq ($(MACHINE),INTLC2DUO)
   include INCLUDE/makefile.c2duointl
endif

########################
# Hitachi              #
########################

ifeq ($(MACHINE),HITACHI)
   include INCLUDE/makefile.hit
endif




######################################################################
#
# Now assemble the libary flags for linking VINE according to
# the variables set above.
#
# Note that /usr/local/lib may not be the correct local library
# directory on some systems. For example, SGI has []/lib, []/lib32
# and []/lib64 for various compilation options. Other systems
# are similar.
#
######################################################################

LIBES= $(LIBGRAPE) $(LIBFFTW) $(LIBIO) $(LIBNATIVE) 
#LIBES= $(LIBGRAPE) $(LIBFFTW) $(LIBIO) $(LIBNATIVE) -lm
LDPATH = -L/usr/local/lib $(LIOPATH) $(LDPATHNAT) $(LDGRAPEPATH)

######################################################################
#
# Now assemble the list of source files for building VINE according to
# the variables set above.
# Some of these modules (source files) are required for operation of 
# the code, those are explicitly specified here. Others are swappable 
# one for another or are removable entirely. They are specified through
# variables which contain the approriate choice according to the make 
# flags set above. The stubs.F file contains templates for routines 
# that are missing so that the code will still compile if some of the 
# *SRCS variables are empty.
#
# SRCS and SRCSF refer to free and fixed form fortran files respectively
#
######################################################################

SRCC = $(G6CSRC)

SRCS= kinds.f90 perform.f90 

SRCSF= dimens.F constants.F stubs.F miscvars.F clmpvars.F \
         partvars.F integvars.F sphvars.F indivtsvars.F treevars.F \
         $(INTEGSRCS) $(SPHSRC) $(PMSRCS) $(PERIODICSRC) $(COSMOSRC) \
         $(SELFFORCESRC) $(PLATSRC) \
         derivcalc.F errorcrit.F indivts.F io.F analyze.F \
         driver.F tree.F treemake.F treesort.F vineutils.F


ifeq ($(SPH),1)
   SRCS  += $(RECIPESSRC)
endif


INITSRCS = kinds.f90 perform.f90 initvine.f90

INITSRCSF = dimens.F constants.F stubs.F miscvars.F clmpvars.F \
            partvars.F integvars.F sphvars.F indivtsvars.F treevars.F \
            io.F \
            $(SPHSRC) $(PMSRCS) $(PERIODICSRC) $(COSMOSRC) $(SELFFORCESRC) \
            $(PLATSRC) \
            tree.F treemake.F treesort.F vineutils.F

ifeq ($(SPH),1)
   INITSRCS  += $(RECIPESSRC)
   INITSRCSF += smoothadjust.F
endif

#-------------------------------------------------------------------
# How to make objects from .F (fixed form) and .f90 (free form) files

.F.o:
	$(FCF) $(FFLAGS) -c $<

%.o: %.f90
	$(FC90) $(F90FLAGS) -c $<


.c.o: 
	cc -O2 -c $<

# dependencies

OBJ  = $(SRCS:.f90=.o)
OBJF = $(SRCSF:.F=.o)

INITOBJ  = $(INITSRCS:.f90=.o)
INITOBJF = $(INITSRCSF:.F=.o)
#-------------------------------------------------------------------
#Make rules for making executables and object files.

$(EXEC): $(OBJ) $(OBJF) 
	$(FCF) $(FFLAGS) $(OBJ) $(OBJF) $(LDPATH) $(LIBES) -o $(EXEC)
	mv $(EXEC) $(HOME)/local/$(ARCH)/bin/


initvine:  $(INITOBJ) $(INITOBJF) 
	$(FCF) $(FFLAGS) $(INITOBJ) $(INITOBJF) $(LDPATH) $(LIBES) -o initvine
	mv initvine $(HOME)/local/$(ARCH)/bin/

writeout:
	echo OBJC         $(OBJC)
	echo SPHSRC       $(SPHSRC)
	echo PMSRCS       $(PMSRCS)
	echo PERIODICSRC  $(PERIODICSRC)
	echo COSMOSRC     $(COSMOSRC)
	echo SELFFORCESRC $(SELFFORCESRC)
	echo DIRSUMSRC    $(DIRSUMSRC)
	echo PLATSRC      $(PLATSRC)

writeoutobj:
	echo OBJC         $(OBJC)
	echo SPHOBJ       $(SPHOBJ)
	echo PMOBJ        $(PMOBJS)
	echo PERIODICOBJ  $(PERIODICOBJ)
	echo COSMOSRC     $(COSMOOBJ)
	echo SELFFORCEOBJ $(SELFFORCEOBJ)
	echo DIRSUMOBJ    $(DIRSUMOBJ)
	echo PLATOBJ      $(PLATOBJ)


.PHONY: clean
clean :
	/bin/rm $(EXEC) *.o *.mod *.MOD


######################################################################
#
# It is an annoying fact of f90 compilers that .mod files that are
# produced have no standard naming format. Some use capital letters
# (MODULE.mod) and some use small letters (module.mod). In order to
# avoid this issue we make some .o files dependent on other .o files
# if they `use' a module. (NB: use is a stronger form of `include'
# which requires compiler interaction at the compile step, in order to
# do various kinds of type checking etc for subroutine/function calls
# (among other things).
# In contrast, object files are only needed at the link step)
#
# It is another annoying fact of f90 compilers and their interaction
# with make that modules often lead to unnecessary compilation cascades.
# So far no one has told the make people, or at least not loudly enough
# to get them to do anything about it.
#
######################################################################

PERIODICOBJ  = $(PERIODICSRC:.F=.o)
SELFFORCEOBJ = $(SELFFORCESRC:.F=.o)
DIRSUMOBJ    = $(DIRSUMSRC:.F=.o)
GRAPEOBJ     = $(GRAPESRC:.F=.o)
INTEGOBJ     = $(INTEGSRCS:.F=.o)
SPHOBJ       = $(SPHSRC:.F=.o)
KERNELOBJ    = $(KERNELSRC:.F=.o)
COSMOOBJ     = $(COSMOSRC:.F=.o)
PMCALCOBJ    = $(PMCALC:.F=.o)
PMOBJ        = $(PMSRCS:.F=.o)
RECIPESOBJ   = $(RECIPESSRC:.f90=.o)

#
# Including the source file on the dependencies line has the nice advantage 
# that if the file is missing you get notified at compile time rather than 
# just finding missing .o files or missing routines at link time 
#

analyze.o    :     analyze.F   kinds.o dimens.o constants.o partvars.o stubs.o
analyze.o    :                 indivtsvars.o miscvars.o derivcalc.o indivts.o 
analyze.o    :                 perform.o $(INTEGOBJ)
clmpvars.o   :    clmpvars.F   kinds.o dimens.o
constants.o  :   constants.F   kinds.o
cosmo.o      :       cosmo.F   kinds.o dimens.o constants.o miscvars.o
derivcalc.o  :   derivcalc.F   kinds.o dimens.o constants.o perform.o stubs.o miscvars.o 
derivcalc.o  :                 indivtsvars.o integvars.o clmpvars.o partvars.o
derivcalc.o  :                 $(PMCALCOBJ) $(INTEGOBJ) $(SPHOBJ) $(PERIODICOBJ) 
derivcalc.o  :                 tree.o treemake.o
dimens.o     :      dimens.F   kinds.o
driver.o     :      driver.F   kinds.o dimens.o constants.o perform.o stubs.o partvars.o 
driver.o     :                 clmpvars.o analyze.o derivcalc.o
driver.o     :                 indivts.o indivtsvars.o io.o miscvars.o 
driver.o     :                 $(INTEGOBJ) integvars.o errorcrit.o
driver.o     :                 vineutils.o treemake.o $(PERIODICOBJ) $(SELFFORCEOBJ)
driver.o     :                 $(PMCALCOBJ) $(COSMOOBJ) $(SPHOBJ) 
energy.o     :      energy.F   kinds.o dimens.o constants.o miscvars.o sphvars.o perform.o 
eostate.o    :     eostate.F   kinds.o dimens.o constants.o miscvars.o sphvars.o perform.o 
errorcrit.o  :   errorcrit.F   kinds.o dimens.o constants.o stubs.o perform.o miscvars.o
errorcrit.o  :                 partvars.o integvars.o $(INTEGOBJ) $(COSMOOBJ) $(SPHOBJ) 
ewald.o      :       ewald.F   kinds.o dimens.o constants.o indivtsvars.o miscvars.o INCLUDE/fftw3.f 
ewald.o      :                 perform.o $(RECIPESOBJ)
forcelaw.o   :    forcelaw.F   kinds.o dimens.o constants.o treevars.o perform.o
forcelaw.o   :                 stubs.o $(GRAPEOBJ) $(DIRSUMOBJ) $(PERIODICOBJ) INCLUDE/hwinfo
forcedirect.o: forcedirect.F   kinds.o dimens.o treevars.o constants.o INCLUDE/hwinfo
grape3.o     :      grape3.F   kinds.o dimens.o constants.o treevars.o indivtsvars.o perform.o miscvars.o
grape5.o     :      grape5.F   kinds.o dimens.o constants.o treevars.o indivtsvars.o perform.o
grape6.o     :      grape6.F   kinds.o dimens.o constants.o treevars.o indivtsvars.o perform.o
indivts.o    :     indivts.F   kinds.o dimens.o constants.o indivtsvars.o miscvars.o perform.o
indivtsvars.o: indivtsvars.F   kinds.o dimens.o
integvars.o  :   integvars.F   kinds.o dimens.o
io.o         :          io.F   kinds.o dimens.o constants.o partvars.o miscvars.o indivtsvars.o
io.o         :                 perform.o vineutils.o clmpvars.o stubs.o $(COSMOOBJ)
io.o         :                 INCLUDE/hwinfo
kinds.o      :       kinds.f90 makefile
miscvars.o   :    miscvars.F   kinds.o dimens.o
leapfrog.o   :    leapfrog.F   kinds.o dimens.o constants.o integvars.o partvars.o miscvars.o
leapfrog.o   :                 perform.o stubs.o $(COSMOOBJ)
partvars.o   :    partvars.F   kinds.o dimens.o
perform.o    :     perform.f90 kinds.o 
pm.o         :          pm.F   kinds.o dimens.o constants.o partvars.o miscvars.o
pm.o         :                 integvars.o indivtsvars.o 
pmcalcs.o    :     pmcalcs.F   kinds.o dimens.o constants.o miscvars.o perform.o
recipes.o    :     recipes.f90 constants.o
rk12.o       :        rk12.F   kinds.o dimens.o constants.o integvars.o partvars.o miscvars.o 
rk12.o       :                 perform.o
sph.o        :         sph.F   kinds.o dimens.o constants.o miscvars.o sphvars.o perform.o 
sph.o        :                 tree.o $(KERNELOBJ)
sphvars.o    :     sphvars.F   kinds.o dimens.o
stubs.o      :       stubs.F   kinds.o dimens.o makefile
tree.o       :        tree.F   kinds.o dimens.o constants.o treevars.o treefuncs 
tree.o       :                 perform.o stubs.o $(SELFFORCEOBJ)
treemake.o   :    treemake.F   kinds.o dimens.o constants.o treevars.o treesort.o treefuncs 
treemake.o   :                 $(SELFFORCEOBJ) perform.o
treesort.o   :    treesort.F   kinds.o dimens.o constants.o
treevars.o   :    treevars.F   kinds.o dimens.o
vineutils.o  :   vineutils.F   kinds.o dimens.o partvars.o indivtsvars.o integvars.o sphvars.o
vineutils.o  :                 treevars.o miscvars.o clmpvars.o tree.o treemake.o 
vineutils.o  :                 perform.o stubs.o $(GRAPEOBJ)
W4kern.o     :      W4kern.F   kinds.o dimens.o constants.o
W4kernalt.o  :   W4kernalt.F   kinds.o dimens.o constants.o


#
# Create source files that may not exist in this directory
#

forcedirect.F:
	if test ! -e forcedirect.F; then                           \
	   if test -e ../../addon1/forcedirect.F; then             \
	      ln -s ../../addon1/forcedirect.F forcedirect.F;      \
	   fi                                                      \
	fi
W4kernalt.F  :
	if test ! -e W4kernalt.F; then                             \
	   if test -e ../../addon2/W4kernalt.F; then               \
	      ln -s ../../addon2/W4kernalt.F W4kernalt.F;          \
	   fi                                                      \
	fi


ifeq ($(FAKE),1)

grape3.o     :               fakegrape.o
grape5.o     :               fakegrape.o
grape6.o     :               fakegrape.o

wait.o       :        wait.F kinds.o
fakegrape.o  :   fakegrape.F kinds.o treevars.o wait.o 

fakegrape.F  :
	if test ! -e fakegrape.F; then                         \
	   if test -e ../../addon1/fakegrape.F; then           \
	      ln -s ../../addon1/fakegrape.F fakegrape.F;      \
	   fi                                                  \
	fi

endif


#
# Problem setup routines 
#

initvine.o     :     initvine.f90 kinds.o dimens.o partvars.o indivtsvars.o clmpvars.o miscvars.o
initvine.o     :                  sphvars.o constants.o treemake.o tree.o io.o smoothadjust.o
smoothadjust.o : smoothadjust.F   kinds.o dimens.o partvars.o indivtsvars.o clmpvars.o miscvars.o
smoothadjust.o :                  constants.o $(SPHOBJ) treemake.o sphvars.o tree.o


